Curves on Frobenius classical surfaces in $\mathbb{P}^3$ over finite fields

In this paper we give an upper bound on the number of rational points on an irreducible curve $C$ of degree $\delta$ defined over a finite field $\mathbb{F}_q$ lying on a Frobenius classical surface $S$ embedded in $\mathbb{P}^3$. This leads us to investigate arithmetic properties of curves lying on surfaces. In a certain range of $\delta$ and $q$, our result improves all other known bounds in the context of space curves.

==> degenerate.tex <==
\jade{Cas : $g'=(y-\tilde y )(x - \tilde x)$ :}

	Suppose that $g'=(y-\tilde{y})/(x-\tilde{x})$. As $y=g(x)$ and $\tilde{y}=g(\tilde{x})$, taking the derivative on both sides gives $g''=0$.
	Let us denote by $p$ the characteristic of the finite field $\Fq$. Then the expansion of the power series $g$  had the following form
	\[g(x)=a_0+a_1 x + \sum_{j \geq 1} a_j x^{jp} + \sum_{j \geq 1}b_j x^{jp+1}.\]
	Now, using that $g'=(y-\tilde{y})/(x-\tilde{x})$, let us prove that $g$ has degree at most 1.
	
	On one hand, its derivative $g'$ can be written 
	\[g'(x)= a_1 + \sum_{j \geq 1}b_j x^{jp}.\] 
	On the other hand, we have
	\[y-\tilde{y}=g(x)-g(\tilde x)=a_1( x- \tilde{x}) + \sum_{j \geq 1} a_j (x^{jp}-\tilde x^{jp}) + \sum_{j \geq 1}b_j (x^{jp+1}-\tilde x^{jp+1}). \]
	Hence, dividing by $x - \tilde x$, we get
		\[g'(x)=a_1 + \sum_{j \geq 1} a_j \left( \sum_{k=0}^{jp-1} x^{jp-1-k}\tilde x^k \right)  + \sum_{j \geq 1}b_j \left(\sum_{k=0}^{jp} x^{jp-k}\tilde x^k \right). \]
		Therefore, 
		\[\sum_{j \geq 1} a_j \left( \sum_{k=0}^{jp-1} x^{jp-1-k}\tilde x^k \right)  + \sum_{j \geq 1}b_j \left(\sum_{k=1}^{jp} x^{jp-k}\tilde x^k \right)=0. \]
		Let us examine the terms of the right handside whose powers are not multiple of $p$. We thus need to explicit $\tilde x$. From Equation \eqref{eq:frob}, there exists $a,b,c \in \overline{\F}_q$ such that
	\[\tilde x=a x^q + b g(x)^q + c u(x,g(x))^q + \tilde x_0,\] 
	where $\tilde{x}_0 \in \overline{\F}_q$ is the $x$-coordinate of the image of the origin under the $q$-Frobenius map. 
